Satisfiability and Synthesis Modulo Oracles

In classic program synthesis algorithms, such as counterexample-guided inductive synthesis (CEGIS), the algorithms alternate between a synthesis phase and an oracle (verification) phase. Many synthesis algorithms use a white-box oracle based on satisfiability modulo theory (SMT) solvers to provide counterexamples. But what if a white-box oracle is either not available or not easy to work with? We present a framework for solving a general class of oracle-guided synthesis problems which we term synthesis modulo oracles. In this setting, oracles may be black boxes with a query-response interface defined by the synthesis problem. As a necessary component of this framework, we also formalize the problem of satisfiability modulo theories and oracles, and present an algorithm for solving this problem. We implement a prototype solver for satisfiability and synthesis modulo oracles and demonstrate that, by using oracles that execute functions not easily modeled in SMT-constraints, such as recursive functions or oracles that incorporate compilation and execution of code, SMTO and SyMO are able to solve problems beyond the abilities of standard SMT and synthesis solvers.

==> figures/dpll.tex <==
\begin{tikzpicture}[>=latex,x=2.3cm,y=1.6cm]

\node[rectangle,draw,minimum height=1cm,minimum width=2.2cm] at (1,4) (dec) {\sc Decide};
\node[rectangle,draw,minimum height=1cm,minimum width=2.2cm] at (1,2) (bcp) {BCP};
\node[rectangle,draw,minimum height=1cm,minimum width=2.2cm] at (2,3) (btr) {\sc BackTrack};
\node[rectangle,draw,minimum height=1cm,minimum width=2.2cm,align=center] at (3,2) (anc) {\sc Analyze\\\sc Conflict};
\node[rectangle,draw,minimum height=1cm,minimum width=2.2cm] at (0,1) (ded) {Deduction};
\node[rectangle,draw,minimum height=1cm,minimum width=2.2cm] at (2,1) (acl) {Add Clauses};
\node[anchor=west] at (3.8,4) (sat) {SAT};
\node[anchor=west] at (3.8,2) (unsat) {UNSAT};

\path[->] ($(bcp.west)+(-0.4,0.15)$) edge ($(bcp.west)+(0,0.15)$);
\path[->] (dec) edge node[below] {all assigned} (sat);
\path[->] (anc) edge (unsat);
\path[->] ($(dec.south)+(-0.15,0)$) edge ($(bcp.north)+(-0.15,0)$);
\path[->] ($(bcp.east)+(0,0.15)$) edge node[above] {conflict} ($(anc.west)+(0,0.15)$);
\path[->] (ded) edge node[above] {theory} node[below] {propagation} (acl);
\draw[->] ($(bcp.west)+(0,-0.15)$) -| ($(ded.north)+(0.15,0)$);
\draw[->] (acl) |- ($(bcp.east)+(0,-0.15)$);
\draw[->] (anc) |- (btr);
\draw[->] (btr) -| ($(bcp.north)+(0.15,0)$);
\draw[->] ($(ded.north)+(-0.15,0)$) |- node[near start,rotate=90,yshift=0.2cm] {nothing to propagate} (dec);

\draw[dashed,color=cyan,very thick,rounded corners] (-0.6,0.6) rectangle (2.6,1.4);
\node[anchor=south west,color=cyan,align=left] at (2.6,0.7) {\bf Theory\\ \bf Solver};

\draw[dotted,color=red!60!black,very thick,rounded corners] (0.3,1.55) rectangle (3.6,4.45);
\node[anchor=north east,color=red!60!black] at (3.7,1.55) {\bf DPLL(T)};

\end{tikzpicture}


==> figures/ogis.tex <==
\begin{tikzpicture}[>=latex,x=3cm,y=2cm]
\node[rectangle,draw,minimum height=0.7cm,minimum width=2.5cm] at (1,1) (s) {{Learner}};
\node[rectangle,draw,minimum height=0.7cm,minimum width=2.5cm] at (1,0) (v) {{Oracles}};
\node[anchor=west] at (1.6,1.1) (ns) {no solution};
\node[anchor=west] at (1.6,0.9) (so) {solution $f^*$};

\path[->] ($(s.west)+(-0.3,0)$) edge ($(s.west)+(0,0)$);
\path[->] (s) edge[above] node {} (ns);
\path[->] (s) edge[above] node {} (so);
\path[->] ($(v.north)+(0.25,0)$) edge[right] node {response} node[left,near start,rotate=90,anchor=base,yshift=0.1cm] {} ($(s.south)+(0.25,0)$);
\path[->] ($(s.south)+(-0.25,0)$) edge[left] node {query} node[right,near start,rotate=270,anchor=base,yshift=0.1cm] {}($(v.north)+(-0.25,0)$);

\end{tikzpicture}

==> macros/macros.tex <==
% \theoremstyle{definition}
% \newtheorem{example}{Example}
% \newcommand{\rem}[1]{\textcolor{red}{[#1]}}
% \newcommand{\ajr}[1]{\rem{#1 --ajr}}








\global\long\def\autobox#1{#1}


\global\long\def\opname#1{\autobox{\operatorname{#1}}}


\global\long\def\dontcare{\_}


\global\long\def\bbracket#1{\left\llbracket #1\right\rrbracket }


\global\long\def\cnot#1{\centernot#1}






\global\long\def\roset#1{\left\{  #1\right\}  }


\global\long\def\ruset#1#2{\roset{#1\;\middle\vert\;#2}}


\global\long\def\union#1#2{#1\cup#2}


\global\long\def\bigunion#1#2{\bigcup_{#1}#2}


\global\long\def\intersection#1#2{#1\cap#2}


\global\long\def\bigintersection#1#2{\bigcap_{#1}#2}


\global\long\def\bigland#1#2{\bigwedge_{#1}#2}


\global\long\def\powerset#1{2^{#1}}




\global\long\def\cart#1#2{#1\times#2}


\global\long\def\tuple#1{\left(#1\right)}


\global\long\def\quoset#1#2{\left.#1\middle/#2\right.}


\global\long\def\equivclass#1{\left[#1\right]}


\global\long\def\refltransclosure#1{#1^{*}}




% \newcommandx\funcapphidden[3][usedefault, addprefix=\global, 1=]{#2#1#3}


\global\long\def\funcapplambda#1#2{\funcapphidden[\,]{#1}{#2}}


\global\long\def\funcapptrad#1#2{\funcapphidden{#1}{\tuple{#2}}}


\global\long\def\funccomp#1#2{#1\circ#2}


\global\long\def\arrow#1#2{#1\to#2}


\global\long\def\func#1#2#3{#1:\arrow{#2}{#3}}




\global\long\def\N{\mathbb{N}}


\global\long\def\Z{\mathbb{Z}}


\global\long\def\Q{\mathbb{Q}}


\global\long\def\R{\mathbb{R}}


\global\long\def\D{\mathbb{D}}


\global\long\def\Zmod#1{\quoset{\Z}{#1\Z}}


\global\long\def\vector#1{\mathbf{#1}}


\global\long\def\dotprod#1#2{#1\cdot#2}


\global\long\def\bool{{\tt bool}}


\global\long\def\true{{\tt true}}


\global\long\def\false{{\tt false}}






\global\long\def\strempty{\epsilon}




\global\long\def\kstar#1{#1^{*}}
\global\long\def\koption#1{#1^{?}}
\global\long\def\kstarn#1#2{#1^{#2}}


\global\long\def\kplus#1{#1^{+}}


\global\long\def\paren#1{{\tt (}#1{\tt )}}


==> macros/sygus-macros.tex <==


\global\long\def\sygus{\left\langle SyGuS\right\rangle }


\global\long\def\cmd{\left\langle Cmd\right\rangle }

\global\long\def\smtcmd{\left\langle SmtCmd\right\rangle }

\global\long\def\oraclecmd{\left\langle OracleCmd\right\rangle }


\global\long\def\setlogiccmd{\left\langle SetLogicCmd\right\rangle }


\global\long\def\sortdefcmd{\left\langle SortDefCmd\right\rangle }


\global\long\def\fundefcmd{\left\langle FunDefCmd\right\rangle }


\global\long\def\vardeclcmd{\left\langle VarDeclCmd\right\rangle }


\global\long\def\fundeclcmd{\left\langle FunDeclCmd\right\rangle }


\global\long\def\synthfuncmd{\left\langle SynthFunCmd\right\rangle }


\global\long\def\constraintcmd{\left\langle ConstraintCmd\right\rangle }
\global\long\def\assumecmd{\left\langle AssumeCmd\right\rangle }


\global\long\def\fundefcmdkwd{\left\langle FunDefCmdKwd\right\rangle }



\global\long\def\checksynthcmd{\left\langle CheckSynthCmd\right\rangle }


\global\long\def\setoptscmd{\left\langle SetOptsCmd\right\rangle }


\global\long\def\symbol{\left\langle Symbol\right\rangle }

\global\long\def\identifier{\left\langle Identifier\right\rangle }
\global\long\def\identifierindex{\left\langle Index\right\rangle }
\global\long\def\qualidentifier{\left\langle QualIdentifier\right\rangle }


\global\long\def\quotedliteral{\left\langle QuotedLiteral\right\rangle }


\global\long\def\sortexpr{\left\langle Sort\right\rangle }


\global\long\def\intconst{\left\langle Numeral\right\rangle }


\global\long\def\realconst{\left\langle Decimal\right\rangle }


\global\long\def\boolconst{\left\langle BoolConst\right\rangle }


\global\long\def\bvconst{\left\langle BVConst\right\rangle }

\global\long\def\hexconst{\left\langle HexConst\right\rangle }
\global\long\def\binaryconst{\left\langle BinConst\right\rangle }

\global\long\def\stringconst{\left\langle StringConst\right\rangle }


\global\long\def\sortedvar{\left\langle SortedVar \right\rangle }
\global\long\def\varbinding{\left\langle VarBinding \right\rangle }


\global\long\def\enumconst{\left\langle EnumConst\right\rangle }


\global\long\def\literal{\left\langle Literal\right\rangle }


\global\long\def\term{\left\langle Term\right\rangle }


\global\long\def\bfterm{\left\langle BfTerm\right\rangle }


\global\long\def\gterm{\left\langle GTerm\right\rangle }


\global\long\def\letterm{\left\langle LetTerm\right\rangle }


\global\long\def\letgterm{\left\langle LetGTerm\right\rangle }


\global\long\def\ntdef{\left\langle GroupedRuleList\right\rangle }

\global\long\def\grammardef{\left\langle GrammarDef\right\rangle }


\global\long\def\feature{\left\langle Feature\right\rangle }

% for datatypes
\global\long\def\dtdec{\left\langle DTDec\right\rangle }
\global\long\def\dtconsdec{\left\langle DTConsDec\right\rangle }


\global\long\def\sortdecl{\left\langle SortDecl\right\rangle }

\global\long\def\option{\left\langle Option\right\rangle }


\global\long\def\fundec{\left\langle FunDec\right\rangle }

\global\long\def\fundef{\left\langle FunDef\right\rangle }

\global\long\def\attribute{\left\langle Attr\right\rangle }

\global\long\def\constdeclkwd{{\tt declare\mbox{-}const}}


\global\long\def\dtdeclkwd{{\tt declare\mbox{-}datatype}}


\global\long\def\dtsdeclkwd{{\tt declare\mbox{-}datatypes}}


\global\long\def\recfundefkwd{{\tt define\mbox{-}fun\mbox{-}rec}}


\global\long\def\recfunsdefkwd{{\tt define\mbox{-}funs\mbox{-}rec}}

\global\long\def\setlogickwd{{\tt set\mbox{-}logic}}
\global\long\def\setlogicinputkwd{{\tt set\mbox{-}logic\mbox{-}input}}
\global\long\def\setlogicoutputkwd{{\tt set\mbox{-}logic\mbox{-}output}}
\global\long\def\setinfokwd{{\tt set\mbox{-}info}}


\global\long\def\sortdefkwd{{\tt define\mbox{-}sort}}

\global\long\def\sortdeclkwd{{\tt declare\mbox{-}sort}}

\global\long\def\fundefkwd{{\tt define\mbox{-}fun}}


\global\long\def\vardeclkwd{{\tt declare\mbox{-}var}}

\global\long\def\primedvardeclkwd{{\tt declare\mbox{-}primed\mbox{-}var}}


\global\long\def\fundeclkwd{{\tt declare\mbox{-}fun}}


\global\long\def\synthfunkwd{{\tt synth\mbox{-}fun}}

\global\long\def\synthinvkwd{{\tt synth\mbox{-}inv}}

\global\long\def\oracledeckwd{{\tt declare\mbox{-}oracle\mbox{-}fun}}

\global\long\def\iooracledeckwd{{\tt oracle\mbox{-}constraint\mbox{-}io}}
\global\long\def\cexoracledeckwd{{\tt oracle\mbox{-}constraint\mbox{-}cex}}
\global\long\def\corroracledeckwd{{\tt declare\mbox{-}correctness\mbox{-}oracle}}
\global\long\def\memoracledeckwd{{\tt oracle\mbox{-}constraint\mbox{-}membership}}
% \global\long\def\dioracledeckwd{{\tt di\mbox{-}oracle}}
\global\long\def\corrcexoracledeckwd{{\tt declare\mbox{-}correctness\mbox{-}cex\mbox{-}oracle}}
\global\long\def\poswitnessoracledeckwd{{\tt oracle\mbox{-}constraint\mbox{-}poswitness}}
\global\long\def\negwitnessoracledeckwd{{\tt oracle\mbox{-}constraint\mbox{-}negwitness}}


% \global\long\def\falsifyoracledeckwd{{\tt declare\mbox{-}oracle\mbox{-}falsify}}



\global\long\def\constraintkwd{{\tt constraint}}
\global\long\def\assumekwd{{\tt assume}}
\global\long\def\constraintinvkwd{{\tt inv\mbox{-}constraint}}

\global\long\def\constraintoraclekwd{{\tt oracle\mbox{-}constraint}}
\global\long\def\assumeoraclekwd{{\tt oracle\mbox{-}assume}}


\global\long\def\checksynthkwd{{\tt check\mbox{-}synth}}


\global\long\def\setoptkwd{{\tt set\mbox{-}option}}

\global\long\def\setoptskwd{{\tt set\mbox{-}options}}


\global\long\def\bitveckwd{{\tt BitVec}}


\global\long\def\arraykwd{{\tt Array}}


\global\long\def\intkwd{{\tt Int}}


\global\long\def\boolkwd{{\tt Bool}}


\global\long\def\enumkwd{{\tt Enum}}


\global\long\def\realkwd{{\tt Real}}

\global\long\def\constantkwd{{\tt Constant}}


\global\long\def\varkwd{{\tt Variable}}


\global\long\def\inputvarkwd{{\tt InputVariable}}


\global\long\def\localvarkwd{{\tt LocalVariable}}


\global\long\def\letkwd{{\tt let}}


\global\long\def\askwd{{\tt as}}

\global\long\def\forallkwd{{\tt forall}}
\global\long\def\existskwd{{\tt exists}}

\global\long\def\truekwd{{\tt true}}
\global\long\def\falsekwd{{\tt false}}

\global\long\def\setfeaturekwd{{\tt set\mbox{-}feature}}

\global\long\def\setfeaturesetkwd{{\tt set\mbox{-}feature\mbox{-}set}}

\global\long\def\fgrammarskwd{{\tt grammars}}
\global\long\def\fquantifierskwd{{\tt quantifiers}}
\global\long\def\ffwddeclskwd{{\tt fwd\mbox{-}decls}}
\global\long\def\frecursionkwd{{\tt recursion}}
\global\long\def\foracleskwd{{\tt oracles}}

% the Boolean sort (not syntax)
\global\long\def\sbool{\mathsf{Bool}}


\global\long\def\slogic{\mathcal{L}}
